PrivImage: Differentially Private Synthetic Image Generation using Diffusion Models with Semantic-Aware Pretraining

Differential Privacy (DP) image data synthesis, which leverages the DP technique to generate synthetic data to replace the sensitive data, allowing organizations to share and utilize synthetic images without privacy concerns. Previous methods incorporate the advanced techniques of generative models and pre-training on a public dataset to produce exceptional DP image data, but suffer from problems of unstable training and massive computational resource demands. This paper proposes a novel DP image synthesis method, termed PRIVIMAGE, which meticulously selects pre-training data, promoting the efficient creation of DP datasets with high fidelity and utility. PRIVIMAGE first establishes a semantic query function using a public dataset. Then, this function assists in querying the semantic distribution of the sensitive dataset, facilitating the selection of data from the public dataset with analogous semantics for pre-training. Finally, we pre-train an image generative model using the selected data and then fine-tune this model on the sensitive dataset using Differentially Private Stochastic Gradient Descent (DP-SGD). PRIVIMAGE allows us to train a lightly parameterized generative model, reducing the noise in the gradient during DP-SGD training and enhancing training stability. Extensive experiments demonstrate that PRIVIMAGE uses only 1% of the public dataset for pre-training and 7.6% of the parameters in the generative model compared to the state-of-the-art method, whereas achieves superior synthetic performance and conserves more computational resources. On average, PRIVIMAGE achieves 30.1% lower FID and 12.6% higher Classification Accuracy than the state-of-the-art method. The replication package and datasets can be accessed online.

==> Sections/final_discussion.tex <==



\section{Discussion}
\label{sec:dis}
This section discusses how \toolname performs without privacy-protective settings, the computational resources required by \toolname, as well as its potential applications and inherent limitations.
We also discuss about how to choose the privacy parameter in Appendix~\ref{ap:epsChoice}.

\subsection{\toolname without Privacy Protection}


This experiment studies how the synthetic performance of \toolname is harmed by adhering to the DP framework. We compared \toolname with three methods: (1) ``NonPrivD'' and ``NonPrivG'' train diffusion models and GANs respectively on the pre-training dataset chosen by \toolname with selection radio 5\%, whereas the gradient in fine-tuning stage and semantic distribution in the pre-training stage are not introduced Gaussian noise. (2) ``NonPriv'' directly uses the sensitive dataset to train the classifier for the downstream classification task. It is noticed that the FID measures the quality of images created by the generative models, so that sensitive datasets do not have an FID value. We conduct these experiments with a privacy budget ($10,1 \times 10^{-5}$).  

Table~\ref{tab:dis1} shows that, on average, \toolnameD and \toolnameG only decrease by 6.5\% and 1.4\% in terms of CA on three classification models. Therefore, with sensitive data protected, \toolname still generates useful synthetic images. In terms of CA, \toolname shows an 11.2\% decrease compared to NonPriv. However, when we increase the generative model size of \toolnameD by 2.2M parameters, the decrease is just 7.9\%. This suggests that more efforts are needed to develop our \toolname further.

\begin{table}[!t]
\vspace{-6.0pt}
\setlength{\tabcolsep}{3pt}
\small
    \centering
    \caption{GPU memory cost, Running time, CA and FID of synthetic images of PDP-Diffusion, DPSDA and \toolname. The time cost of SQF includes the time taken to train SQF and to use the trained SQF for querying the semantic distribution.}
    \begin{tabular}{l|c|c|c|c}
    \toprule
      \multicolumn{2}{c|}{Evaluation Metrics}& PDP-Diffusion & DPSDA & \toolname\\
    \hline
    \multirow{4}{*}{Memory} & Pre-train &  107GB & 0GB & 55GB \\
     & Fine-tune & 158GB & 0GB & 89GB\\
     & SQF & 0GB & 0GB & 22GB\\
     & Synthesis & 177GB & 219GB & 83GB\\
     \hline
    \multirow{4}{*}{Time} & Pre-train  & 87h & 0h & 46h\\ %-66\%
     & Fine-tune  & 24h & 0h & 3h\\ %-99\%
     & SQF  & 0h & 0h & 9h\\
     & Synthesis & 0.37h & 12h & 0.15h\\
     \hline
     \multirow{3}{*}{CA (\%)} & LR & 15.07 & 14.3 & 33.11 \\
     & MLP & 14.17 & 13.4 & 36.78\\
     & CNN & 24.27 & 15.1 & 70.91\\
    \hline
    \multicolumn{2}{c|}{FID} & 22.90 & 16.2 & 21.69\\
    \bottomrule
\end{tabular}
\label{tab:computationalResource}
\vspace{-8.0pt}
\end{table}


\subsection{Consumption of Computational Resource}
\label{subsec:ComputationalResource}

% \begin{table}[!t]
% \vspace{-6.0pt}
% \setlength{\tabcolsep}{3pt}
% \small
%     \centering
%     \caption{GPU memory cost, Running time, CA and FID of synthetic images of PDP-Diffusion and \toolname. `Changes' represents the relative percentage variation in the evaluation metrics of \toolname when compared to PDP-Diffusion. }
%     \begin{tabular}{l|c|c|c|c}
%     \toprule
%       \multicolumn{2}{c|}{Evaluation Metrics}& PDP-Diffusion & \toolname & Changes \\
%     \hline
%     \multirow{4}{*}{Memory} & Pre-train &  107GB & 55GB & \multirow{4}{*}{\textbf{-50\%}}\\
%      & Fine-tune & 158GB & 89GB &\\
%      & SQF & 0 & 22GB &\\
%      & Synthesis & 177GB & 83GB &\\
%      \hline
%     \multirow{4}{*}{Time} & Pre-train  & 87h& 46h & \multirow{4}{*}{\textbf{-48\%}}\\ %-66\%
%      & Fine-tune  & 24h& 3h &\\ %-99\%
%      & SQF  & 0 & 9h &\\
%      & Synthesis & 22min & 9min &\\
%      \hline
%      \multirow{3}{*}{CA (\%)} & LR & 15.07 & 33.11 & \textbf{+18.0}\\
%      & MLP & 14.17 & 36.78 & \textbf{+22.6}\\
%      & CNN & 24.27 & 70.91 & \textbf{+46.6}\\
%     \hline
%     \multicolumn{2}{c|}{FID} & 22.90 & 21.69 & \textbf{-5\%} \\
%     \bottomrule
% \end{tabular}
% \label{tab:computationalResource}
% \vspace{-8.0pt}
% \end{table}


This section presents the high efficiency of \toolname and the significant trade-off between the computation resource cost and synthesis performance. We trained the state-of-the-art method PDP-Diffusion using an 80M diffusion models~\cite{dpdm-sota} and \toolnameD using a 6.1M diffusion model on {\tt CIFAR-10}. We also implement DPSDA~\cite{api} using a 270M diffusion model pre-trained on {\tt ImageNet}. We compare their GPU memory usage and time cost during pre-training, fine-tuning and synthesis on identical computational configurations. \toolname needs additional time to train the SQF.

Table~\ref{tab:computationalResource} shows that \toolname uses only 50\% and 59\% of the GPU memory used by PDP-Diffusion and DPSDA, respectively. In terms of runtime, \toolname is 48\% faster than PDP-Diffusion. These results can be attributed to the compact dataset selected by \toolname for pre-training and lighter generative models that \toolname uses. Although \toolname requires more time compared to DPSDA, the majority of \toolname's time is spent on training, while the synthesis process is 98\% faster than DPSDA. When our synthesis method needs to respond to multiple queries, DPSDA could be significantly slower than \toolname.
% Pre-training PDP-Diffusion on the entire public dataset requires a diffusion model with 80M parameters, while \toolname only uses 5\% of the public dataset to pre-train lightly-parameterized diffusion model with only 6.1M parameters. 
Despite the significant savings in computational resources, our \toolname still achieves an FID and average CA that are 5\% lower and 29\% higher than PDP-Diffusion.



As presented in Table~\ref{tab:rq1}, compared to an 1.8M model, PDP-Diffusion with an 80M model does achieve better FID. However, the average CA on three classifiers drops by 5.7\%, suggesting that the synthetic images are less useful. This is attributed to the fact that the $l_2$-norm of the noise added during DP-SGD scales linearly to the dimension of parameters, leading to a ``curse of dimensionality'' and making the training of generative models unstable~\cite{dpdm,nolargemodel1,nolargemodel2}. We also conduct another experiment to prove this ``curse of dimensionality'' and put the result in Appendix~\ref{ap:OMI}. Besides, we may need to upload our sensitive data to a remote server using such over-parameterized models, presenting potential security concerns~\cite{DPPublicPretraining1}. Therefore, we should be more concerned about achieving great synthesis with lightly parameterized models, which are less affected by DP-SGD and can be used on end-user devices more easily.



% \kc{for the fair comparison, we train all Diffusion-based methods (e.g., DPDM, PDP-Diffusion, and \toolnameD) using the same diffusion model with 1.8M parameters. Using such light models, PDP-Diffusion cannot generate synthetic images with great utility and fidelity for large pre-training dataset they use. In this paper, we more concern about how to achieve great synthesis with lightly-parameterized models, which are less affected by DP-SGD and can be employed on end-user devices more easily. It is expensive to employ PDP-Diffusion with 80M models as they proposes. Besides, even though PDP-Diffusion uses diffusion models with 80M parameters, our \toolnameD can still achieve competitive or even better results. For example, \toolnameD achieves 7.6\% and 19.1\% lower FID with 4M and 6.1M parameters respectively. Therefore, it is not meaningful to choose PDP-Diffusion with 80M models as our baselines.}


\subsection{Applications and Limitations}

This subsection discusses the application scope and limitations of \toolname.

\noindent \textbf{Potential Applicability to Other Fields.} Though this paper primarily focuses on image data synthesis, we posit that \toolname has high potential applicability to other data types, such as text data. Numerous studies have highlighted the effectiveness of diffusion models in tasks like text generation~\cite{diffusionText1} and audio synthesis~\cite{diffusionAudio1}. Analogous to the practical adopted in \toolname, by judiciously selecting a suitable public dataset as well as integrating pre-training with fine-tuning methodologies, it seems feasible to achieve DP text, audio synthesis, and even other fields.

\noindent \textbf{Dependence on Public Data.} The primary advantage of \toolname lies in its ability to query the semantic distribution of sensitive data and subsequently select data from a public dataset that closely aligns with the sensitive dataset for pre-training. However, when the distribution of the public data substantially deviates from that of the sensitive data, \toolname faces limited opportunities to pick out such pertinent data. In the absence of a suitable public dataset, the effectiveness of \toolname in generating complex image datasets while adhering to the DP guarantee diminishes.


% \subsection{Real-World Application Scenarios}

% \toolname can produce synthetic images of exceptional fidelity and utility using compact generative models with just \textbf{1.8M} parameters. Furthermore, it leverages a minimal pre-training dataset consisting of merely \textbf{13K} images. Such efficiency and compactness make \toolname highly suitable for deployment on a plethora of end-user devices. This obviates the necessity to transfer sensitive data to remote cloud services, enhancing user privacy and data security. \toolname lets organizations use and share synthetic images without privacy worries, aiding the creation of strong machine learning models without compromising data privacy.
% \tw{feel this can be deleted}
% \tw{you can put some limitations here, e.g., we assume sensitive dataset must be within imagenet and cannot handle strange datasets}


==> Sections/final_exp_setup.tex <==

\begin{table}[!t]
\vspace{-7.0pt}
\small
    \centering
    \caption{Data split of three datasets used in our experiments.}
    \label{tab:DataSplit}
    \begin{tabular}{l|ccc}
    \toprule
    \diagbox{Dataset}{Subset}& Training& Validation& Test\\
    \hline
    {\tt CIFAR-10}& 45,000 & 5,000&10,000\\
    {\tt CelebA}& 162,770 & 19,867&19,962\\
    {\tt ImageNet}& 1,281,167 & 50,000& 100,000\\
    \hline
\end{tabular}
\end{table}

\section{Experiment Setup}
\label{sec:experiment_setup}

This section details the experimental settings to evaluate the proposed \toolname, including the investigated datasets, baselines, evaluation metrics, and implementation.

\subsection{Investigated Datasets}
\label{subsec:dataset}
We utilize ImageNet, a widely used dataset for pre-training in computer vision, along with CelebA and CIFAR-10 for DP image synthesis research. These sensitive datasets, featuring over 200K celebrity images and 60,000 natural images across 10 classes respectively, offer a greater synthesis challenge compared to the commonly used MNIST and FashionMNIST. All datasets are divided into a training set, a validation set, and a test set. Please refer to Table~\ref{tab:DataSplit} for details. All images in {\tt CelebA} undergo center-cropping and are subsequently resized to dimensions of 64×64 and 32×32, which are named {\tt CelebA32} and {\tt CelebA64} respectively. Figure 10 presents examples of {\tt ImageNet}, {\tt CIFAR-10}, and {\tt CelebA}, and We present more details in Appendix D.1 in our full version~\cite{privimage}.



\subsection{Baselines}
\label{subsec:baselines}
This paper selects DPDM~\cite{dpdm}, PDP-Diffusion~\cite{dpdm-sota}, DP-LDM~\cite{dpldm}, DPSDA~\cite{api}, DPGAN~\cite{dpsgd-gan3,dpsgd-gan8,dpsgd-gan9} and DPGAN with pre-training (DPGAN-p) as our baselines, which follow the same framework of DP image synthesis proposed in Section~\ref{subsec:framework}. All these baselines are trained with state-of-the-art image generative models, GANs and diffusion models, and incorporate DP-SGD~\cite{dpsgd} to ensure the protection of sensitive datasets. Additionally, PDP-Diffusion, DP-LDM, DPSDA and DPGAN-p leverage the public dataset for pre-training.

% \noindent \textbf{GS-WGAN:} The GS-WGAN model, as presented in the work of~\cite{dpsgd-gan2,dpsgd}. To regulate the sensitivity of the model during this process, the GS-WGAN leverages the properties of the Wasserstein distance~\cite{wgan}. Adopting the Wasserstein distance provides a more stable gradient flow, ensuring that the sanitized generator produces high-quality outputs while adhering to differential privacy constraints.

\begin{itemize}[leftmargin=*]

\item  \textbf{DPDM:} DPDM~\cite{dpdm} trains diffusion models with lightweight parameters and a substantial number of images (e.g., `batch sizes') at each training iteration. To protect the sensitive dataset, Gaussian noise is introduced to the gradient of the diffusion model, aligning with the DP-SGD methodology~\cite{dpsgd}.

\item \textbf{PDP-Diffusion:} PDP-Diffusion~\cite{dpdm-sota} adopts a training approach that capitalizes on larger batch sizes to enhance the stability and convergence speed of the model training. By leveraging the public dataset, the model benefits from a broader knowledge base, potentially improving its subsequent fine-tuning on the sensitive dataset.

\item \textbf{DP-LDM:} Given a pre-trained diffusion model, DP-LDM~\cite{dpldm} proposes to fine-tune only its label embedding module and attention module. This approach reduces the number of trainable parameters and requires less noise to achieve the same privacy budget.

\item \textbf{DPSDA:} DPSDA~\cite{api} proposes a Private Evolution algorithm that progressively guides the pre-trained models to generate a synthetic image dataset similar to the sensitive one without the need for fine-tuning.

\item \textbf{DPGAN:} DPGAN~\cite{dpsgd-gan3,dpsgd-gan8,dpsgd-gan9} represents a typical method that trains GAN with DP-SGD for sensitive data synthesis. We refer to the implementation of~\cite{dpsgd-gan8}, which is the sole work offering executable code along with privacy analysis. 
% We substituted their network architectures with one of the most efficient GANs -- BigGAN~\cite{biggan}.

\item \textbf{DPGAN-p:} To validate the effectiveness of dataset as selected by \toolname, we introduce an additional baseline, DPGAN-p. Building upon DPGAN, DPGAN-p first pre-trains the GAN on the public dataset, and subsequently fine-tunes it on the sensitive dataset adopting the pre-training method proposed by~\cite{dpdm-sota}.

\end{itemize}

Recently, PDP-Diffusion~\cite{dpdm-sota} with 80M parameters has achieved SOTA results on {\tt CIFAR-10}~\cite{cifar10} under $\varepsilon=10$.
For the dataset {\tt CIFAR-10}, we set $\delta$ to $10^{-5}$, and for {\tt CelebA}, we set it to $10^{-6}$. We adopt three privacy budgets, $\varepsilon=\{10,5,1\}$, for both datasets. These specific privacy budgets have been commonly used in prior DP image synthesis research~\cite{dpdm,dpdm-sota}.
\toolname prioritizes efficient image synthesis using low-parameterized neural networks even under smaller privacy budgets 5 and 1, saving substantial computation resources and achieving superior results.

\subsection{Evaluation Metrics}
\label{subsec:metrics}
We evaluate the fidelity and utility of the synthetic dataset using two widely accepted metrics: Fr\'{e}chet Inception Distance (FID) and Classification Accuracy, as commonly employed in prior research~\cite{dpdm,dpdm-sota,dpsgd-gan8}.

\noindent \textbf{Fr\'{e}chet Inception Distance (FID):} FID is a metric widely used to assess the fidelity of images generated by Generative models~\cite{ddpm,ddim,ddpm_song,biggan}. A lower FID suggests that the generated images are higher quality and more akin to the real ones. We generate 5,000 synthetic images to calculate FID.

\noindent \textbf{Classification Accuracy (CA):} We assess the utility of synthetic images with specific attributes or categories in the accuracy of downstream classification. Specifically, we select three classification models: Logistic Regression (LR), Multi-Layer Perceptron (MLP), and Convolutional Neural Network (CNN). These models are trained on synthetic datasets using different methods and their classification accuracy is tested on the sensitive test dataset. We generate 50,000 synthetic images to train classifiers.

\noindent \textbf{Semantic Distribution Similarity (SDS):} This paper proposes a metric to access the semantic distribution similarity between two image datasets. Let $D_1$ and $D_2$ be the two image datasets with semantics of $\left\{ {s_1^j} \right\}_{j = 1}^{N{S_1}}$ and $\left\{ {s_2^j} \right\}_{j = 1}^{N{S_2}}$ respectively, where $NS_1$ and $NS_2$ represent the number of semantics in their respective images. The semantic distribution similarity of $D_1$ and $D_2$ is calculated as, 

\begin{equation}
\label{eq:sds}
    SDS\left( {{D_1},{D_2}} \right) = \sum\limits_{i = 1}^{N{S_1}} {\sum\limits_{k = 1}^{N{S_2}} {w_1^iw_2^k\frac{{V(s_1^i) \cdot V(s_2^k)}}{{\left\| {V(s_1^i)} \right\|\left\| {V(s_2^k)} \right\|}}} }
\end{equation}
where $V$ indicates a function that converts a semantic or a word into its embedding vector~\cite{glove}. Besides, ${\frac{{V(s_1^i) \cdot V(s_2^k)}}{{\left\| {V(s_1^i)} \right\|\left\| {V(s_2^k)} \right\|}}}$ calculates the cosine similarity of the embedding vector of $s_1^i$ and $s_2^k$. The ${w_1^i}$ represents the frequency of semantic $s_1^i$ in $D_1$, and we consider semantics with higher frequency can better represent the dataset. The higher value of $SDS(D_1,D_2)$ suggests that $D_1$ and $D_2$ have closer semantic distribution.


\subsection{Implementation}
\label{sub:Imp}

All image generative methods are realized with Python 3.8 on a server with 4 NVIDIA GeForce A100 and 512GB memory. 

We replicate DPDM~\cite{dpdm} using open-source implementation repositories, and building upon that, we also reproduce PDP-Diffusion~\cite{dpdm-sota}. In particular, we use a larger batch size and pre-train the diffusion models on {\tt ImageNet}~\cite{imagenet}. For DP-LDM~\cite{dpldm}, we follow their proposed approach and fine-tune only the label embedding and attention modules in the diffusion models, keeping the other parameters frozen. We replicate DPSDA~\cite{api} using their open-source code and replace their RANDOM-API with the pre-trained diffusion model used in PDP-Diffusion for a fair comparison. To ensure fairness, we discuss the comparison with their 270M diffusion models in Section~\ref{subsec:ComputationalResource}. For DPGAN~\cite{dpsgd-gan8}, we refer to the practice adopted for GAN training with gradient sanitizing released in opacus\footnote{https://github.com/pytorch/opacus/tree/main/examples}. Our implementation of DPGAN-p is based on DPGAN, incorporating similar training techniques as suggested in PDP-Diffusion~\cite{dpdm-sota}. 

For \toolname, we choose diffusion models and GANs as the image generative models within our \toolname framework. We refer to these two variations as \toolnameD and \toolnameG, respectively. For the fair comparison, all Diffusion-based and GAN-based methods use lightly parameterized models with the same parameters. Although PDP-Diffusion proposes to use large-scale diffusion models (e.g. with 80M parameters), we believe this way is ineffective for both the synthesis performance and computational resource saving, which are discussed in Section~\ref{subsec:ComputationalResource} in more details. We recommend readers refer to Appendix D in our full version~\cite{privimage} for more implementation details.

% Additionally, we establish three other baselines: Non-private G, Non-private D, and NonPriv. Non-private G and Non-private D represent the optimal versions of \toolnameG and \toolnameD, respectively, \kc{ and gradient of models.  For NonPriv, the synthetic images are the original sensitive images.}



==> Sections/final_methodology.tex <==
\section{Methodology}
\label{sec:method}

% Several methods have been proposed to achieve DP image synthesis on some naive image datasets~\cite{dpsgd-gan1,dpsgd-gan2,dpsgd-gan3,dpsgd-gan4,dpsgd-gan6,dpsgd-gan7,dpsgd-gan8,dpsgd-gan9,dpdm,dp2vae,dp-mepf,lvae}, like MNIST~\cite{mnist} and FashionMNIST~\cite{fmnist}, which contains only gray images. To achieve DP image synthesis on more colorful dataset, such as CIFAR-10~\cite{cifar10} and CelebA~\cite{celeba}, some studies propose to pre-train the generative model~\cite{CVPretaining1,CVPretaining2,CVPretaining3} with a public dataset~\cite{dpdm-sota,dpldm,api,dp-merf}.  DP-MERF~\cite{dp-merf} trains a feature extractor neural network using public data and use the trained feature extractor to query the mean feature embedding of the sensitive dataset. The query results are privatized based on the Gaussian Mechanism~\cite{gm}. Finally, they train a image generator to generate synthetic dataset whose mean feature embedding is pushed close to the queried embedding. DPSDA~\cite{api} propose to leverage available foundation models, which are usually some image generative models trained on public datasets and published online others. However, when foundation models are not available or the public datasets and the sensitive dataset differ a lot, DPSDA are not effective compared to existing methods~\cite{api}. DP-LDM~\cite{dpldm} leverage Latent Diffusion Models~\cite{ldm}, which consists of an encoder, a decoder and a diffusion module. They pre-train the encoder and decoder on the public dataset and fine-tune the whole model on the sensitive dataset with gradient sanitized by Gaussian noise~\cite{dpsgd}.

% Recently, DP-Diffusion~\cite{dpdm-sota} achieves SOTA results on the dataset CIFAR-10~\cite{cifar10} and Camelyon17~\cite{camelyon1,camelyon2}. Compared to DP-LDM, they propose to pre-train the whole diffusion model on the public dataset and fine-tune the pre-trained model on the sensitive dataset. Since the public dataset is usually large, such as ImageNet~\cite{imagenet} which contains more than 1 million images, they need to use models with more parameters, which are usually over-parameterized for the sensitive dataset, to obtain well pre-trained models. In the experiments of~\cite{dpdm-sota} on CIFAR-10~\cite{cifar10}, the number of parameters is over 80 mililion. For example, in our experiment, a diffusion model with only 1 million parameters still can achieve good synthesis performance under a non-private setting.
% 然后介绍一下这几个用了public data的方法



This paper focuses on exploring how to leverage the public dataset for more effective pre-training and proposes a novel DP image synthesis method, \toolname. We divide \toolname into three steps. Initially, we utilize the semantic labels from the public dataset to derive a semantic query function. Then, this function aids in querying the semantic distribution of the sensitive dataset, facilitating data selection for pre-training. Finally, we initiate pre-training of an image generative model using the selected data and then fine-tune this model on the sensitive dataset using DP-SGD.
% \tw{i wrote we made the observation about the importance of distribution similarities between pertaining and fine-tuning. can we say something (better with evaluation results) here? basically, you need to motivate why using semantic queries}
\begin{figure}[!t]
    \centering
    \setlength{\abovecaptionskip}{0pt}
    \includegraphics[width=1.0\linewidth]{Figures/method/semantic_show.pdf}
    \caption{Two images with their captions. The same and different semantics two images own are in \textcolor[RGB]{0,165,79}{green} and \textcolor[RGB]{238,29,35}{red} respectively. Although the two images differ a lot in pixel, they have the same semantics, \textit{\textbf{\textcolor[RGB]{0,165,79}{man}}} and \textit{\textbf{\textcolor[RGB]{0,165,79}{dog}}}.}
    \label{fig:semantic_show}
\end{figure}

\subsection{Motivation}
\label{sec:motivation}

Studies indicate that if there is minimal overlap between the distributions of pre-training and target dataset (which is the sensitive dataset in our studied problem), the effectiveness of pre-training diminishes~\cite{DPPublicPretraining1,DPPublicPretraining2,DPPublicPretraining3}. Therefore, drawing inspiration from this understanding, we select the data that is ``similar'' to sensitive data from the public dataset for the pre-training of generative models to develop the DP image synthesis method. We select semantic distribution as a metric to gauge the similarity between the two datasets and provide our rationale for this choice as follows.

Semantics provide a high-level representation of images and have played a prominent role in various computer vision studies~\cite{Semantic1,Semantic2,Semantic3}. As illustrated in Figure~\ref{fig:semantic_show}, image semantics refers to the meaning and interpretation derived from an image. Unlike low-level features, such as color, texture, and edges that can be directly extracted from the image, semantics capture the “meaning” or “content” of an image, which often requires higher-level processing and understanding~\cite{Semantic4,Semantic5}. 
Most public image datasets have their semantic labels, like caption~\cite{COCOCaption}, object~\cite{COCODetection}, and category~\cite{imagenet}. 
Since our focus is on generating low-resolution images, which typically have simple content (e.g., each {\tt CIFAR-10} image contains only a single object), we propose utilizing the category labels of the public dataset to query the semantic distribution of the sensitive dataset. This information can then be used to select more relevant data for pre-training. 





\subsection{Query Image Semantics}
\label{subsec:qis}

% \subsubsection{Image Semantics}
% \label{sec:image_semnatics}

% Semantics provide a high-level representation of images and have played a prominent role in various computer vision studies~\cite{Semantic1,Semantic2,Semantic3}. As illustrated in Figure~\ref{fig:semantic_show}, image semantics refers to the meaning and interpretation derived from an image. Unlike low-level features, such as color, texture, and edges that can be directly extracted from the image, semantics capture the “meaning” or “content” of an image, which often requires higher-level processing and understanding~\cite{Semantic4,Semantic5}. Most public image datasets have their semantic labels, like caption~\cite{COCOCaption}, object~\cite{COCODetection}, and category~\cite{imagenet}. We propose to leverage the semantic labels of the public dataset to query the semantic distribution of the sensitive dataset, which can be used to select more useful data for pre-training.

% Semantics provide a high-level image description, making it more comprehensible for humans. If we can extract semantic information from the sensitive dataset in a manner that conforms to DP, then we can leverage this queried semantic information to select appropriate pre-training data from the public dataset. 
We aim to derive a semantic query function that takes an image as input and returns its semantics. In this study, we use the category labels from the public dataset to represent the semantics of sensitive images. The objective while training a semantic query function $Q$ is to minimize the difference between the predicted semantic labels and the true labels. This is achieved by minimizing a loss function $\mathcal{L}_Q$, e.g., the Cross-Entropy loss~\cite{CrossEntropy}, which is defined as,

\begin{equation}
\label{eq:L_Q}
    {\mathcal{L}_Q}: = {\mathbb{E}_{\left( {x,\ {s}} \right)\sim {D_p}}}\left[ {\sum_{i = 1}^{NS} { - {s_i}\log {Q_i}\left( x \right)} } \right]
\end{equation}
where $D_p$ is the public dataset. Each pair in $D_p$ consists of an image $x$ and its semantics labels $s$. $NS$ indicates the number of possible semantics in $D_p$. $s_i = 1$ indicates that the image has the $i$-th semantic label, whereas $s_i = 0$ denotes the absence of this semantic. $Q_i(x)$ is a scalar value between 0 and 1, representing the probability that image $x$ is associated with the semantic $s_i$, as determined by the semantic query function $Q$. Through minimizing Eq.~\eqref{eq:L_Q}, we train the semantic query function $Q$ to extract semantics from images. 

After training, for each sensitive image, the semantic query function $Q$ can predict the probability that the image has the $i$-th semantic $s_i$.  Given that each image potentially can have multiple semantic labels, we select the top-$k_1$ probable semantics as predicted by $Q$ to represent the semantics of the input-sensitive image, where $k_1$ is a hyper-parameter. A higher $k_1$ suggests considering a greater number of semantics in images. 
% As illustrated in Figure~\ref{fig:semantic_show}, \kc{one} image could involve multiple semantics. We aim for the semantic query function $Q$ to characterize the input image with richer and more meaningful semantics. To achieve this, we select the top-$k$ probable semantics as predicted by $Q$ to represent the semantics of the input-sensitive image.

\begin{figure}[!t]
    \centering
    \setlength{\abovecaptionskip}{0pt}
    \includegraphics[width=1.0\linewidth]{Figures/method/sdq.png}
    \caption{An example of using the semantic query function to retrieve the semantic distribution from the sensitive dataset. We first train the semantic query function using the public dataset. This function is used to obtain the semantic distribution of the sensitive dataset. To ensure privacy, we then incorporate the Gaussian noise into our query results.}
    \label{fig:sdq}
\end{figure}

\subsection{Semantic Distribution Query}
\label{subsec:sdq}
\toolname aims to select data from the public dataset for pre-training, ensuring its semantic distribution is similar to that of the sensitive dataset, without revealing any sensitive information. Towards this goal, after querying the semantics of each piece of sensitive data, this section delves into constructing a semantic distribution $SD$ for the sensitive dataset. Given that the number of semantics from the public dataset is constant, it intuitively follows that we can represent the semantic distribution as the frequency distribution of semantics derived from the sensitive dataset. Specifically, $SD$ can be conceptualized as a dictionary where the keys represent the semantics of the public dataset and the values denote the frequency of each semantic within the sensitive dataset. To safeguard the privacy of the sensitive dataset, as presented in Theorem~\ref{the:sd}, we introduce Gaussian noise to the retrieved semantic distribution, in line with the RDP (which is described in Theorem~\ref{the:rdp4sgm}), ensuring the query results adhere to differential privacy.


\begin{theorem}
    \label{the:sd}
    The semantic distribution $SD$ has global sensitivity $\Delta_{SD}=\sqrt{k_1}$, where $k_1$ is the number of semantics we query from each sensitive image. For any $\alpha>1$, incorporating noise $\mathcal{N}\left( {0,k_1{\sigma_2 ^2} {\rm I}} \right)$ into the semantic distribution $SD$ makes the query results satisfies ($\alpha$, $\alpha /\left( {2\sigma _2^2} \right)$-RDP.
    % (2) Publishing semantic distribution $SD$ with noise $\mathcal{N}\left( {0,2k\ln \frac{{1.25}}{\delta }/\varepsilon^2{\rm{I}}} \right)$ satisfies ($\varepsilon, \delta$)-DP.
\end{theorem}
We put the proof of Theorem~\ref{the:sd} in Appendix F in our full version~\cite{privimage}. After obtaining the sensitive semantic distribution, a straightforward way is to select data from the public dataset to obtain a pre-training dataset whose semantic distribution is close to the sensitive one. However, since the sensitive semantic distribution is noisy for incorporating the Gaussian noise, it is ineffective to focus on the semantics with low frequency, which is more easily affected by the added noise. Therefore, we focus on the semantics with high frequency. Specifically, we select the top-$k_2$ semantics based on their probabilities in the semantic distribution to represent the semantic description of the sensitive dataset. 
Finally, the public data, whose semantics are included in the semantic description queried from the sensitive dataset, are selected for pre-training. Our method ensures that all semantics of the selected pre-training data fall within the high-probability regions of the sensitive semantic distribution.
% \kc{Besides, we set $k_1=k_2=k$ in following contents, which means that we use the same $k$ for semantic query in Section~\ref{subsec:qis} and semantic selection.}
We put detailed analysis in Appendix~\ref{ap:sqs}. 

We provide an example to help readers better understand the processes of semantic query and the selection of a pre-training dataset. As shown in Figure \ref{fig:sdq}, each image in the public dataset is labeled with a semantic tag, either \emph{bee} or \emph{zebra}. We first train the semantic query function using the public dataset, then determine the semantics of sensitive images using this trained function. We set $k_1=1$ and $k_2=1$, implying that each sensitive image considers only one semantic. The initial query results yield $\{zebra:3,bee:0\}$ (although the sensitive data contains horses, zebra is the closest label from $Q$).  To ensure privacy, we introduce Gaussian noise to these results, resulting in a modified output of $\{zebra:2.7,bee:1.5\}$. Given that $k_2=1$, we select the semantic \emph{zebra}, which has the highest frequency among all semantic candidates, as the representative descriptor of the sensitive dataset. Ultimately, we select only those public images labeled as \emph{zebra} for our pre-training. In a word, we select pre-training data from the public dataset guided by the perturbed semantic distribution of the sensitive dataset.

Considering applying our method for conditional generation, where the sensitive dataset has been divided into several subsets with corresponding categories, we query a semantic distribution for each subset. This query still satisfies Theorem~\ref{the:sd} because each sensitive image only provides an independent prediction. Therefore, we can label the selected image with the category of the sensitive subset it belongs to. For example, the selected samples can be zebras or, in unfortunate cases, birds from {\tt ImageNet}, but we label them as horses and pre-train our model accordingly.


% \begin{algorithm}[!t]
% 	\caption{Fine-tuning with Gradient Sanitizing}
% 	\label{alg:fine-tuning}
% 	\textbf{Input}: Sensitive dataset $D_s$; Image generative model $G$ parameterized by $\theta$; Objective of generative models: $\mathcal{L}$; Batch size $B$; Learning rate $\eta$; Scale coefficient $C$; Gaussian variance $\sigma_1^2$; Max iterations $T_m$\\
%     $T \leftarrow 0$\\
%     \While{$T<T_m$}{
%         Randomly sample the the image training batch $x_{1:B}$ from $D_s$ \\
%         \tcp{Calculate gradient}
%         $g_{1:B} \leftarrow {{\nabla _\theta } \mathcal{L} \left( {{G_\theta }\left( {{x_{1:B}}} \right)} \right)}$\\
%         \tcp{Scale gradient}
%         ${g_{1:B}}^\prime  \leftarrow \min \left\{ {1,\frac{C}{{{{\left\| {{g_{1:B}}} \right\|}_2}}}} \right\}{g_{1:B}}$\\
%         \tcp{Add Gaussian noise}
%         $\hat g \leftarrow \frac{1}{B}\sum\limits_{i = 1}^B {{g_i}^\prime }  + \frac{{\sigma_1 C}}{B}e,e\sim \mathcal{N} \left( {0,{\rm{I}}} \right)$\\
%         \tcp{Update parameter}
%         $\theta  \leftarrow \theta  - \eta \hat g$\\
%         $T \leftarrow T+1$\\
%     }
%     \textbf{Output}: The well-trained image generative model: $G^\ast$\\
% \end{algorithm}


\subsection{Pre-training and Fine-tuning}
\label{subsec:pf}

\begin{algorithm}[!t]
	\caption{Fine-tuning with Gradient Sanitizing}
	\label{alg:fine-tuning}
	\textbf{Input}: Sensitive dataset $D_s$; Image generative model $G$ parameterized by $\theta$; Objective of generative models: $\mathcal{L}$; Batch size $b$; Learning rate $\eta$; Clip coefficient $C$; Gaussian variance $\sigma_1^2$; Max iterations $T_m$\\
    $T \leftarrow 0$\\
    \While{$T<T_m$}{
        Randomly sample the the image training batch $x_{1:b}$ from $D_s$ \\
        \tcp{Calculate gradient}
        $g_{1:b} \leftarrow {{\nabla _\theta } \mathcal{L} \left( {{G_\theta }\left( {{x_{1:b}}} \right)} \right)}$\\
        \tcp{Scale gradient}
        ${g_{1:b}}^\prime  \leftarrow \min \left\{ {1,\frac{C}{{{{\left\| {{g_{1:b}}} \right\|}_2}}}} \right\}{g_{1:b}}$\\
        \tcp{Add Gaussian noise}
        $\hat g \leftarrow \frac{1}{b}\sum\limits_{i = 1}^b {{g_i}^\prime }  + \frac{{\sigma_1 C}}{b}e,e\sim \mathcal{N} \left( {0,{\rm{I}}} \right)$\\
        \tcp{Update parameter}
        $\theta  \leftarrow \theta  - \eta \hat g$\\
        $T \leftarrow T+1$\\
    }
    \textbf{Output}: The well-trained image generative model: $G^\ast$\\
\end{algorithm}

We pre-train the image generative models on the selected dataset and subsequently fine-tune these pre-trained models on the sensitive dataset. 
% We train the generative models during the pre-training stage using Stochastic Gradient Descent (SGD)~\cite{sgd}. 
In particular, in the fine-tuning phase, we use DP-SGD~\cite{dpsgd} to update the model in adherence to the DP framework, ensuring the protection of sensitive dataset's privacy. Next, we explain how to apply standard DP-SGD works in our fine-tuning in Algorithm~\ref{alg:fine-tuning}.

As described in Algorithm~\ref{alg:fine-tuning}, let $\mathcal{L}$ be the training objective of generative models (e.g., Eq.~\eqref{eq:L_DM} and~\eqref{eq:L_GAN}) and we want to minimize $\mathcal{L}$ through updating the parameters $\theta$ of our neural network $G_{\theta}$. At each training iteration, we first compute the gradient ${g = {{\nabla _\theta } \mathcal{L}\left( {{G_\theta }\left( {x} \right)} \right)}}$, where $x$ is an input image. 
% \tw{acknowledge the equation and alg1 are standard dp-sgd applied to  our setting}
Then, we clip the gradient for controlling the maximal $l_2$-norm of every gradient, like $g' = \min \left\{ {1,\frac{C}{{{{\left\| g \right\|}_2}}}} \right\} g$, where $C$ is a hyper-parameter. Lastly, we introduce Gaussian noise with variance $\sigma_1^2$ to the scaled gradient. In a word, we update the $G_\theta$ with the noisy gradient, which is defined as,
\begin{equation}
\label{eq:dpsgd}
    \hat g = \frac{1}{b}\sum\limits_{i = 1}^b {\min \left\{ {1,\frac{C}{{{{\left\| {{g_i}} \right\|}_2}}}} \right\}{g_i}}  + \frac{{\sigma_1 C}}{b}e,\;\; e\sim \mathcal{N} \left( {0,{\rm{I}}} \right),
    \nonumber
\end{equation}
\noindent {where $b$ is the batch size. Given privacy budget $\varepsilon$ and $\delta$, the maximal training iterations are constrained by the predetermined privacy budget $\varepsilon$ and $\delta$.}

\begin{algorithm}[!t]
	\caption{\toolname Workflow}
	\label{alg:privimage}
	\textbf{Input}: Public dataset $D_p$ with its semantics label $S_p$; Sensitive dataset $D_s$; Semantic query function $Q$ parameterized by $\phi$; Image generative model $G$ parameterized by $\theta$; Semantics query parameters $k_1,k_2$; Gaussian variance $\sigma_2^2$ for Semantic Distribution ($SD$); Privacy budget $\varepsilon$ and $\delta$.\\
	
    \tcp{Obtain semantic query function}
    Train $Q_\phi$ on $D_p$ and $S_p$ with Eq.~\eqref{eq:L_Q}\label{alg2:l2}\\
    \tcp{Query semantic distribution}
    Initiate the semantic distribution $SD$ $\leftarrow {{\rm O}_{NS \times 1}}$\label{alg2:l3}\\
    \For{$x \in D_s$}{\label{alg2:l4}
		Query $k_1$ semantics $\left[ {{s_1}, \cdots {s_{k_1}}} \right]$ from $Q\left( x \right)$\label{alg2:l5}\\
		\For{$s \in \left[ {{s_1}, \cdots {s_{k_1}}} \right]$}{\label{alg2:l6}
            Obtain the index j of $s$\label{alg2:l7}\\
            $SD\left[ j \right] +  = 1$\label{alg2:l8}
        }\label{alg2:l9}
	}\label{alg2:l10}
    $SD = SD + \mathcal{N} \left( {0,k_1{\sigma_2 ^2}{\rm{I}}} \right)$\label{alg2:l11}\\
    Semantic description $S^* \leftarrow$ top-$k_2$ semantics in $SD$\label{alg2:l12}\\
    \tcp{Choose data from the public dataset}
    Selected dataset $D_{ps} \leftarrow \varnothing$\label{alg2:l13}\\
    \For{$(x, s_p) \in D_p$}{\label{alg2:l14}
            \If{$s_p \in S^*$}{\label{alg2:l15}
			$D_{ps} = x \cup D_{ps}$\label{alg2:l16}
		}\label{alg2:l17}
	}\label{alg2:l18}
    \tcp{Pre-train and fine-tune $G_\theta$}
    Pre-train $G_\theta$ on $D_{ps}$\label{alg2:l19}\\
    % Obtain Gaussian variance $\sigma_1^2$ through Theorem~\ref{the:obtainSigma} \label{alg2:l20}\\
    % Fine-tune $G_\theta$ on $D_{s}$ following Algorithm~\ref{alg:fine-tuning}\label{alg2:l21}\\
    Fine-tune $G_\theta$ on $D_{s}$ following Algorithm~\ref{alg:fine-tuning}\label{alg2:l21}\\
    Generate $D_s^*$ by leveraging $G_\theta$\label{alg2:l22}\\
    \textbf{Output}: Synthetic dataset $D_s^*$\label{alg2:l23}\\
\end{algorithm}

% \tw{i feel this statement belongs to our methodology or at least next paragraph (we can say, we advocate a smaller model because xx); do we have experiments on large vs small models?}
A previous study has proved that model size scales sublinearly with data size~\cite{modelDataSize}. To achieve good pre-training on such large datasets, we tend to use models with larger parameters. In contrast, these models can often be over-parameterized when applied to the sensitive dataset. Whereas, we recommend to train models with fewer parameters. This is because more parameters indicate higher dimension of gradient. When the $l_2$-norm of gradient is constrained by clipping, the value of each gradient dimension decreases with the increase of the dimension. Consequently, the gradient becomes more susceptible to perturbations from consistent Gaussian noise, resulting in unstable training of generative models. Thus, it is preferable to train lightly parameterized generative models rather than over-parameterized ones~\cite{dpdm,nolargemodel1,nolargemodel2}. Moreover, with the reduction in the size of the pre-training dataset, \toolname enables us to well train generative models with fewer parameters during the pre-training and fine-tuning stages, thereby benefiting the efficiency of training.



Algorithm~\ref{alg:privimage} elaborates the process for \toolname, which produces a synthetic dataset of fidelity and utility similar to the sensitive dataset without privacy leakage. First, we train a semantic query function on a public dataset with Eq.~\eqref{eq:L_Q} (Line~\ref{alg2:l2}). Then, we use the trained semantic query function to query the semantic distribution of the sensitive dataset (Lines~\ref{alg2:l3}-\ref{alg2:l10}). After adding Gaussian noise to the query results (Line~\ref{alg2:l11}), we use it to select data from the public dataset for pre-training a generative model (Line~\ref{alg2:l12}-\ref{alg2:l19}). 
% Then, we obtain the Gaussian variance for gradient sanitizing through Theorem~\ref{the:obtainSigma} (Line~\ref{alg2:l20}) and 
Then, we fine-tune the generative model on the sensitive dataset with DP-SGD (Line~\ref{alg2:l21}). Finally, the fine-tuned model generates a synthetic image dataset (Line~\ref{alg2:l22}).  

The privacy analysis of \toolname is put into Appendix F in our full version~\cite{privimage}. In particular, in \toolname, two processes consume the privacy budget: (1) querying the semantic distribution of the sensitive dataset and (2) querying the gradient during each training iteration while fine-tuning on the sensitive dataset. Both these processes can be viewed as compositions of multiple Sub-sampled Gaussian Mechanism (SGM) instances~\cite{sgm}. Therefore, we use RDP described in Theorem~\ref{the:rdp4sgm} to track the privacy budget cost of \toolname.



% \subsection{\kc{Privacy Analysis}}
% In \toolname, two processes consume the privacy budget: (1) querying the semantic distribution of the sensitive dataset and (2) querying the gradient during each training iteration while fine-tuning on the sensitive dataset. Both these processes can be viewed as compositions of multiple Sub-sampled Gaussian Mechanism (SGM) instances~\cite{sgm}. As explained in Theorem~\ref{the:rdp4sgm}, we utilize RDP to monitor the privacy cost throughout these processes. Typically, we set the training iterations $T_m$ and sample ratio (or batch size) $q$ before we train our models. Therefore, we need to choose a proper Gaussian variance $\sigma_2^2$ for gradient sanitizing to make \toolname satisfy ($\varepsilon, \delta$)-DP.
% Specifically, given sensitive images sampling ratio $q$, training iterations $T_m$, Gaussian variance $\sigma_2^2$ for semantic distribution query and privacy budget ($\varepsilon,\delta$), the Gaussian standard deviation $\sigma_1$ can be obtained through,
% \begin{theorem}
% \label{the:obtainSigma}
%     Given sensitive images sampling ratio $q$, training iterations $T_m$ and Gaussian variance $\sigma_2^2$ for semantic distribution query, \toolname satisfies ($\varepsilon, \delta$)-DP with Gaussian variance $\sigma_1^2$ for gradient sanitizing, where $\sigma_1 = \mathop {\arg \min }\limits_{{\sigma _1}} {\left[ {\varepsilon  - \mathop {\min }\limits_\alpha  \left( {T_m {\gamma _F}\left( {\alpha ,{\sigma _1},q} \right) + \frac{\alpha }{{2\sigma _2^2}} - \frac{{\log \left( \delta  \right)}}{{\alpha  - 1}}} \right)} \right]^2}$.
% \end{theorem}

% \noindent Where ${\gamma _F}\left( {\alpha ,{\sigma _1},q} \right)$ represents the RDP each training iteration consumes and can be calculated through Eq.~\eqref{eq:rdp_gamma}. 
% Detailed proof of Theorem~\ref{the:obtainSigma} can be found in Appendix~\ref{ap:pa}.\tw{the section title is `Budget Allocation'. but the section is really only about privacy proof (passive tracking not actively allocating). perhaps discuss how much to spend on queries (can refer to evaluation results)}



==> Sections/final_rq.tex <==
% \begin{table}[!t]
% \vspace{-5.0pt}
% \setlength{\tabcolsep}{3pt}
% \small
%     \centering
%     \caption{FID and CA of \toolname and four baselines on {\tt CIFAR-10}~\cite{cifar10}, {\tt CelebA32} and {\tt CelebA64}~\cite{celeba} with $\varepsilon=10$. Best performance in each column is highlighted. }
%     \label{tab:rq1}
%     \begin{tabular}{l|cccc|c|c}
%     \toprule
%     \multirow{3}{*}{Method} & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CelebA32} & {\tt CelebA64 }\\
%     \Xcline{2-7}{0.5pt}
%     & \multicolumn{3}{c}{CA (\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID}\\
%      \Xcline{2-4}{0.5pt}
%      & LR & MLP & CNN & &\\
%     \hline
%     DPGAN
% & 9.17 & 8.4  & 10.5  & 258 & 202 & 121 \\
%     DPGAN-p 
% & 13.6 & 14.9  & 24.1 & 49.7& 29.7 & 51.1 \\
%     DPDM 
% & 20.7 & 24.6  & 21.3 & 304 & 113 & 115 \\
%     PDP-Diffusion  
% & 18.7 & 21.4 & 30.4 & 66.8& 22.6 & 51.6\\
%     \hline
%     \rowcolor{gray0} \toolnameG 
% & 19.9 & 24.5 & 44.3  & 28.1& \textbf{18.9} & \textbf{38.2} \\
%     \rowcolor{gray0} \toolnameD & \textbf{32.6} & \textbf{36.5}  & \textbf{68.8} & \textbf{27.6} & 19.1 & 49.3 \\
%     \bottomrule
% \end{tabular}
% \vspace{-8.0pt}
% \end{table}

\begin{table*}[!t]
\vspace{-5.0pt}
\setlength{\tabcolsep}{2.6pt}
\small
    \centering
    \caption{FID and CA of \toolname and four baselines on {\tt CIFAR-10}~\cite{cifar10}, {\tt CelebA32} and {\tt CelebA64}~\cite{celeba} with $\varepsilon=10,5,1$. For space limitation, {\tt CeA32} and {\tt CeA64} refer to {\tt CelebA32} and {\tt CelebA64} respectively. The best performance in each column is highlighted using the bold font.}
    \label{tab:rq1}
    \begin{tabular}{l|cccc|c|c|cccc|c|c|cccc|c|c}
    \toprule
    \multirow{4}{*}{Method} & \multicolumn{6}{c|}{$\varepsilon=10$} & \multicolumn{6}{c|}{$\varepsilon=5$} & \multicolumn{6}{c}{$\varepsilon=1$}\\
    \Xcline{2-19}{0.5pt}
    & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CeA32} & {\tt CeA64} & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CeA32} & {\tt CeA64} & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CeA32} & {\tt CeA64}\\
    \Xcline{2-19}{0.5pt}
    & \multicolumn{3}{c}{CA(\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multicolumn{3}{c}{CA(\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multicolumn{3}{c}{CA(\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID}\\
     \Xcline{2-4}{0.5pt} \Xcline{8-10}{0.5pt} \Xcline{14-16}{0.5pt}
     & LR & MLP & CNN & & & & LR & MLP & CNN & & & & LR & MLP & CNN & &\\
    \hline
    DPGAN & 9.17 & 8.4  & 10.5  & 258 & 202 & 121 & 14.2 & 14.6 & 13.0 & 210 & 227 & 190 & 16.2 & 17.4 & 14.8 & 225 & 232 & 162\\
    DPGAN-p & 13.6 & 14.9  & 24.1 & 49.7& 29.7 & 51.1 & 13.9 & 14.3 & 19.2 & 48.5 & 23.9 & 52.2 & 11.3 & 13.8 & 12.8 & 70.1 & 37.9 & 54.5\\
    DPDM & 20.7 & 24.6  & 21.3 & 304 & 113 & 115 & 21.1 & 24.7 & 22.0 & 311 & 122 & 127 & 19.6 & 22.3 & 14.7 & 340 & 223 & 243\\
    DP-LDM & 15.2 & 14.1 & 26.0 & 48.6 & 21.9 & 58.0 & 15.3 & 14.6 & 24.8 & 48.9 & 22.2 & 63.9 & 12.8 & 11.8 & 18.8 & 50.1 & 45.5 & 131.9\\
    PDP-Diffusion & 18.7 & 21.4 & 30.4 & 66.8& 22.6 & 51.6 & 19.3 & 22.2 & 28.7 & 70.0 & 23.6 & 55.9 & 17.7 & 19.4 & 22.9 & 87.5 & 33.7 & 77.7\\
    DPSDA & 24.1 & 25.0 & 47.9 & 29.9 & 23.8 & 49.0 & 23.5 & 24.4 & 46.1 & 30.1 & 33.8 & 49.4 & 24.2 & 23.6 & 47.1 & 31.2 & 37.9 & 54.9\\
    \hline
    \rowcolor{gray0} \toolnameG & 19.9 & 24.5 & 44.3  & 28.1& \textbf{18.9} & \textbf{38.2} & 19.6 & 24.6 & 39.2 & 29.9 & \textbf{19.8} & \textbf{45.2} & 15.8 & 18.0 & 25.5 & 47.5 & 31.8 & \textbf{45.1}\\
    \rowcolor{gray0} \toolnameD & \textbf{32.6} & \textbf{36.5}  & \textbf{68.8} & \textbf{27.6} & 19.1 & 49.3 & \textbf{32.4} & \textbf{35.9} & \textbf{69.4} & \textbf{27.6} & 20.1 & 52.9 & \textbf{30.2} & \textbf{33.2} & \textbf{66.2} & \textbf{29.8} & \textbf{26.0} & 71.4\\
    \bottomrule
\end{tabular}
\end{table*}

\begin{figure*}[!t]
    \centering
    % \setlength{\abovecaptionskip}{0cm}
    \includegraphics[width=0.95\linewidth]{Figures/RQ1/tsne_0331.png}
    \caption{The t-SNE visualizations depict the embedding distribution of the synthetic images using four DP dataset synthetic methods within the {\tt CIFAR-10} dataset with $\varepsilon=10$. We obtain embeddings by using CNN classifiers trained on synthetic images.}
    \label{fig:tsne}
        \vspace{-4.0pt}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \setlength{\abovecaptionskip}{0pt}
%     \includegraphics[width=1\linewidth]{Figures/RQ1/cifar10_sample_comp.png}
%     \caption{Examples of Synthetic {\tt CIFAR-10}~\cite{cifar10} images with $\varepsilon=10$. These generative models are trained using our tools \toolnameD, as well as PDP-Diffusion~\cite{dpdm-sota} and DPGAN-p. Each row corresponds to a category from the {\tt CIFAR-10} dataset. }
%     \label{fig:cifar10_comp_show}
%     \vspace{-4.0pt}
% \end{figure*}

\section{Evaluation Results}
\label{sec:rq}
% This section addresses four research questions (RQs) to evaluate the effectiveness of \toolname. Specifically, we investigate (1) whether \toolname generates higher-quality images than the baselines, (2) reasons why the queried semantic distribution improves fine-tuning, (3) performance of \toolname under a constrained privacy budget\tw{can we merge (3) with (1)?}, and (4) impact of hyper-parameters on \toolname.
This section addresses three research questions (RQs) to evaluate the effectiveness of \toolname. Specifically, we investigate (1) whether \toolname generates higher-quality images than the baselines, (2) reasons why the queried semantic distribution improves fine-tuning, and (3) impact of hyper-parameters on \toolname.



\subsection*{RQ1. How effective is \toolname for synthesizing useful images?}


\noindent \textbf{Experiment Design.} We explore whether \toolname can generate synthetic images with higher fidelity and utility than baselines. We compare our \toolnameG and \toolnameD (which is described in Section~\ref{sub:Imp}) with six baselines introduced in Section~\ref{subsec:baselines} on {\tt CIFAR-10}~\cite{cifar10} and {\tt CelebA}~\cite{celeba} under the privacy budget $\varepsilon=\{10,5,1\}$.


\noindent \textbf{Result Analysis.} Table~\ref{tab:rq1} shows that \toolname outperforms all baselines in terms of the FID and CA of downstream classification tasks using synthetic images on {\tt CIFAR-10}, {\tt CelebA32} and {\tt CelebA64} across three distinct privacy budgets. 
% \kc{Conditional {\tt CelebA} generation results are put into Appendix~\ref{ap:conditionalCelebA}.}

When $\varepsilon=10$, for {\tt CIFAR-10}, \toolnameG and \toolnameD outperform all the baselines in terms of FID with specifically 7.7\% lower than the SOTA method DPSDA~\cite{api}, suggesting that the fidelity of images generated by \toolname more closely aligns with the sensitive dataset. For the utility of synthetic images, \toolnameD achieves superior downstream classification accuracy on all three classification models with especially \textbf{20.9\%} higher than the SOTA method~\cite{api} on the CNN classifier. \toolnameG outperforms all GAN-based baselines and DPDM~\cite{dpdm}, achieving competitive results with the SOTA method. \toolnameG outperforms all the baselines in terms of FID with specifically 13.7\% and 22.0\% lower than the SOTA method on {\tt CelebA32} and {\tt CelebA64}, which implies that our \toolname is also effective when there is a substantial difference between the public and sensitive dataset.
Although \toolnameD does not achieve a lower FID than DPSDA on {\tt CelebA64}, we consider a practical advantage of \toolnameD to be its ability to directly sanitize the diffusion model. Once the model is well-trained, \toolname can respond to any number of synthesis queries with fast speed while still protecting data privacy due to the post-processing property~\cite{dp}. In contrast, DPSDA incurs the same significant time cost for each synthesis query, as discussed in Section~\ref{subsec:ComputationalResource}. Moreover, their privacy analysis cannot ensure the security of multiple synthesis queries.

For privacy budget 5 and 1, \toolname consistently surpasses all baselines. Particularly, as $\varepsilon$ shifts from 10 to 1, the FID of synthetic {\tt CIFAR-10} images produced by \toolnameD and \toolnameG drops only by 7.8\% and 7.2\%. In contrast, the FID for the state-of-the-art method diminishes by 23.7\%, and for DPGAN-p, it decreases by a substantial 41.0\%. For {\tt CelebA32} and {\tt CelebA64}, \toolnameD and \toolnameG only decreases by 36.1\% and 18.1\% respectively, while the SOTA method decreases by 49.1\% and 50.6\%. However, our \toolnameG decreases by 68.2\% on {\tt CelebA32}. It is well known that GAN suffers from unstable training~\cite{wgan}. Increased gradient noise due to a restricted privacy budget can further intensify this instability. Hence, we believe diffusion models might be more appropriate as image generative models in scenarios with limited privacy budgets.

\begin{figure*}[t]
    \centering
    \setlength{\abovecaptionskip}{0pt}
    \includegraphics[width=0.96\linewidth]{Figures/RQ1/cifar10_sample_comp.png}
    \caption{Examples of Synthetic {\tt CIFAR-10}~\cite{cifar10} images with $\varepsilon=10$. These generative models are trained using our tools \toolnameD, as well as PDP-Diffusion~\cite{dpdm-sota} and DPGAN-p. Each row corresponds to a category from the {\tt CIFAR-10} dataset. }
    \label{fig:cifar10_comp_show}
    \vspace{-4.0pt}
\end{figure*}


Additionally, we investigate the distribution characteristics of the synthetic dataset to validate the high utility of our generated data. Specifically, we first use trained CNN classifiers from the dataset generated by \toolnameD, PDP-Diffusion, DPSDA, and DPGAN-p, to undertake the classification task within the {\tt CIFAR-10}. With the aid of the well-trained CNN, each image is transformed into an embedding vector. This vector encapsulates the most pertinent feature information utilized by the CNN for classification. We use t-SNE to visualize them in a two-dimension space. Figure~\ref{fig:tsne} illustrates that embeddings of image data from \toolnameD are projected into 10 clusters aligning with 10 categories. This suggests that the classifier adeptly discerns the unique features of images, thereby achieving superior performance compared to the CNNs trained on the dataset provided by other methods. In contrast, dataset embeddings from others do not form distinct clusters, leading their classifiers to struggle with classification.
Examples of synthetic images for {\tt CIFAR-10} from various methods are presented in Figure~\ref{fig:cifar10_comp_show}. Additionally, we present more synthetic images for {\tt CelebA} and {\tt Camelyon17}~\cite{camelyon1} in Appendix G.1 in our full version~\cite{privimage}.


\begin{table}[h]
\vspace{-8.0pt}
\setlength{\tabcolsep}{3pt}
    \centering
    \renewcommand\arraystretch{1}
    \begin{tabular}{p{0.95\columnwidth}}
    \Xhline{1.0pt}
         \rowcolor{gray0} \noindent \textbf{Answers to RQ1}: Synthetic images produced by \toolname exhibit greater fidelity and utility compared to all baseline methods with three distinct privacy budgets. On average, the FID of the synthetic dataset is \textbf{6.8\%} lower, and the CA of the downstream classification task is \textbf{13.2\%} higher, compared to the state-of-the-art method.\\
    \Xhline{1.0pt}
    \end{tabular}
\vspace{-8.0pt}
\end{table}


% \noindent \textbf{Answers to RQ1}: Synthetic images produced by \toolname exhibit greater fidelity and utility compared to all baseline methods. On average, the FID of the synthetic dataset is \textbf{29.8\%} lower, and the CA of the downstream classification task is \textbf{14.3\%} higher, compared to the state-of-the-art method. 


\subsection*{RQ2. How do the semantic distribution queries of \toolname improve the fine-tuning?}

\begin{figure}[t]
\vspace{+5.0pt}
    \centering
    \includegraphics[width=0.97\linewidth]{Figures/RQ2/rq2_gc.pdf}
    \caption{(Left) The FID of baselines pre-trained on the entire public dataset and ours \toolname pre-trained on the selected public dataset.
    (Right) The SDS between the sensitive dataset and different pre-training datasets.}
    \label{fig:rq2}
            \vspace{-4.0pt}
\end{figure}


\noindent \textbf{Experiment Design.} We conducted experiments to explore whether the fine-tuning of generative models is enhanced by leveraging our proposed semantic distribution query to select images from the entire public dataset for pre-training. As a result, \toolname can synthesize images with greater fidelity and utility. We approach this from two perspectives: data distribution similarity and semantic distribution similarity. To evaluate data distribution similarity, we compute the FID of synthetic images generated by different methods, where generative models have only been pre-trained and not fine-tuned on the sensitive dataset. To evaluate semantic distribution similarity, we assess the SDS (as given in Eq.~\eqref{eq:sds}) between the sensitive dataset and the pre-training dataset across various selection ratios. Additionally, we present a showcase from the pre-training dataset selected by our \toolname, to further verify the semantic distribution similarity from a visual perspective in Appendix G.2 in our full version~\cite{privimage}.

% \begin{table*}[!t]
% \vspace{-5.0pt}
% \small
%     \centering
%     \caption{The FID and CA on {\tt CIFAR-10}~\cite{cifar10} and {\tt CelebA}~\cite{celeba} with smaller privacy budget $\varepsilon=5$ and $\varepsilon=1$. We highlight the best performance in each row using bold font.}
%     \label{tab:rq3}
%     \begin{tabular}{l|cccc|c|c|cccc|c|c}
%     \toprule
%     \multirow{4}{*}{Method} & \multicolumn{6}{c|}{$\varepsilon=5$} & \multicolumn{6}{c}{$\varepsilon=1$}\\
%     \Xcline{2-13}{0.5pt}
%     & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CelebA32} & {\tt CelebA64} & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CelebA32} & {\tt CelebA64}\\
%     \Xcline{2-13}{0.5pt}
%     & \multicolumn{3}{c}{CA(\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multicolumn{3}{c}{CA(\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID}\\
%      \Xcline{2-4}{0.5pt} \Xcline{8-10}{0.5pt}
%      & LR & MLP & CNN & & & & LR & MLP & CNN & &\\
%     \hline
%     DPGAN & 14.2 & 14.6 & 13.0 & 210 & 227 & 190 & 16.2 & 17.4 & 14.8 & 225 & 232 & 162\\
%     DPGAN-p & 13.9 & 14.3 & 19.2 & 48.5 & 23.9 & 52.2 & 11.3 & 13.8 & 12.8 & 70.1 & 37.9 & 54.5\\
%     DPDM & 21.1 & 24.7 & 22.0 & 311 & 122 & 127 & 19.6 & 22.3 & 14.7 & 340 & 223 & 243\\
%     PDP-Diffusion & 19.3 & 22.2 & 28.7 & 70.0 & 23.6 & 55.9 & 17.7 & 19.4 & 22.9 & 87.5 & 33.7 & 77.7\\
%     \hline
%     \rowcolor{gray0} \toolnameG & 19.6 & 24.6 & 39.2 & 29.9 & \textbf{19.8} & \textbf{45.2} & 15.8 & 18.0 & 25.5 & 47.5 & 31.8 & \textbf{45.1}\\
%     \rowcolor{gray0} \toolnameD & \textbf{32.4} & \textbf{35.9} & \textbf{69.4} & \textbf{27.6} & 20.1 & 52.9 & \textbf{30.2} & \textbf{33.2} & \textbf{66.2} & \textbf{29.8} & \textbf{26.0} & 71.4\\
%     \bottomrule
% \end{tabular}
% \end{table*}

\begin{figure*}[!t]
    \centering
    \setlength{\abovecaptionskip}{0pt}
    \includegraphics[width=0.98\linewidth]{Figures/RQ4/rq4_gc.pdf}
    \caption{The two left figures present the effect of the selection ratio on the FID of the synthesized image dataset and the CA for downstream classification tasks. The models are trained on datasets selected from the public dataset for pre-training, using various selection ratios. "100\%" represents that pre-training generative models on the entire public dataset. The right two figures display the effect of model size, where the selection ratios are set as 5\% and 1\% for {\tt CIFAR-10} and {\tt CelebA} respectively.}
    \label{fig:rq4}
    \vspace{-4.0pt}
\end{figure*}

\noindent \textbf{Result Analysis.} We analyze our results from two similarity between the synthesized and sensitive dataset as follows. 

\noindent \textit{Data Distribution Similarity.} The left panel of Figure~\ref{fig:rq2} presents that when generative models are pre-trained on the selectively curated public dataset, \toolname produces datasets with superior FID results compared to baselines pre-trained on the entire public dataset. Before fine-tuning on the sensitive dataset, \toolname can intuitively generate synthetic images with a data distribution closer to the sensitive data than images produced by existing methods. \textit{\toolname wins at the beginning.} With an equal number of fine-tuning iterations, \toolname still achieves superior performance.

\noindent \textit{Semantic Distribution Similarity.} For the {\tt CIFAR-10} dataset~\cite{cifar10}, we adopt its 10 category labels as its semantic representation. Similarly, for the {\tt CelebA} dataset~\cite{celeba}, we use its 40 face attribute labels to represent its semantics. The public dataset {\tt ImageNet}~\cite{imagenet} is characterized by its 1000 category labels. We experiment with various selection ratios from this public dataset by adjusting the number of queried semantics, $k_2$, as described in Section~\ref{subsec:sdq}. The right panel of Figure~\ref{fig:rq2} displays that the semantic distribution similarity between {\tt ImageNet}~\cite{imagenet} and {\tt CIFAR-10}\cite{cifar10} surpasses that of {\tt CelebA}\cite{celeba}, aligning with our human visual perceptions as presented in Figure 10 in our full version~\cite{privimage}, indicating the utility of our proposed SDS metric. The datasets selected by our \toolname exhibit a closer semantic distribution to the two sensitive datasets than the entire public dataset across different selection ratios. Leveraging the semantic distribution query, \toolname selects a pre-training dataset whose semantic distribution closely mirrors that of the sensitive dataset, all while operating within a minimal privacy budget.


\begin{table}[H]
\vspace{-8.0pt}
\setlength{\tabcolsep}{3pt}
    \centering
    \renewcommand\arraystretch{1}
    \begin{tabular}{p{0.95\columnwidth}}
    \Xhline{1.0pt}
         \rowcolor{gray0} \noindent \textbf{Answers to RQ2}: \toolname selects a pre-training dataset that resembles the sensitive data more closely than the entire public data. Before fine-tuning the sensitive dataset, \toolname produces synthetic images with a data distribution maligned with the sensitive data. As a result, \toolname delivers enhanced DP image synthesis.\\
    \Xhline{1.0pt}
    \end{tabular}
\vspace{-8.0pt}
\end{table}


% \noindent \textbf{Answers to RQ2}: \toolname selects a pre-training dataset that more closely resembles the sensitive data than the entire public data. Before fine-tuning on the sensitive dataset, PRIVIMAGE produces synthetic images that have a data distribution maligned with the sensitive data. As a result, \toolname delivers enhanced DP image synthesis.



% \subsection*{RQ3. How does \toolname perform under stringent privacy budgets?}

% \noindent \textbf{Experiment Design.} This experiment evaluates \toolnameG and \toolnameD against the four baselines. The evaluations are conducted under stringent privacy budgets: ($\varepsilon=5$, $\delta=10^{-5}$) and ($\varepsilon=1$, $\delta=10^{-5}$). Our test datasets include {\tt CIFAR-10}~\cite{cifar10} and {\tt CelebA}~\cite{celeba}.



% \noindent \textbf{Result Analysis.} Table~\ref{tab:rq3} reveals that even with these reduced privacy budgets, \toolname consistently surpasses all baselines. As $\epsilon$ shifts from 10 to 1, the FID of synthetic {\tt CIFAR-10} images produced by \toolnameD and \toolnameG drops only by 7.8\% and 7.2\%. In contrast, the FID for the state-of-the-art method diminishes by 23.7\%, and for DPGAN-p, it decreases by a substantial 41.0\%. For {\tt CelebA32} and {\tt CelebA64}, \toolnameD and \toolnameG only decreases by 36.1\% and 18.1\% respectively, while the SOTA method decreases by 49.1\% and 50.6\%. However, our \toolnameG decreases by 68.2\% on {\tt CelebA32}. It is well known that GAN suffers from unstable training~\cite{wgan}. Increased gradient noise due to a restricted privacy budget can further intensify this instability. Hence, we believe Diffusion models might be more appropriate as image generative models in scenarios with limited privacy budgets.

% \begin{table}[h]
% \vspace{-8.0pt}
% \setlength{\tabcolsep}{3pt}
%     \centering
%     \renewcommand\arraystretch{1}
%     \begin{tabular}{p{0.95\columnwidth}}
%     \Xhline{1.0pt}
%          \rowcolor{gray0} \noindent \textbf{Answers to RQ3}: Even under tight privacy budgets, \toolname can produce valuable synthetic images and surpasses current methods. On average, when $\varepsilon=5$ and $1$, the FID of the synthetic dataset is \textbf{28.9\%} and \textbf{31.7\%} lower, and the CA of downstream classification task is \textbf{11.9\%} and \textbf{11.5\%} higher, compared to the SOTA method.\\
%     \Xhline{1.0pt}
%     \end{tabular}
% \vspace{-8.0pt}
% \end{table}


\subsection*{RQ3. How do hyper-parameters affect the performance of \toolname?}


% \begin{table}[!t]
%     \centering
%     \caption{Impact of selection ratio on \toolnameG on CelebA~\cite{celeba}.}
%     \label{rq4:table1}
%     \begin{tabular}{c|cc}
%     \toprule
%     Selection Ratio  & CelebA32 & CelebA64\\
%     \hline
%     1\% & 18.87 & 38.16\\
%     5\% & 20.33 & 39.07\\
%     10\% & 21.28 & 42.04\\
%     20\% & 19.81 & 43.20\\
%     50\% & 22.02 & 38.65\\
%     \bottomrule
% \end{tabular}
% \end{table}
% \begin{table}[!t]
%     \centering
%     \caption{Impact of selection ratio on \toolnameD on {\tt CIFAR-10}~\cite{cifar10}.}
%     \label{rq4:table2}
%     \begin{tabular}{c|cccc}
%     \toprule
%     Selction Ratio & FID & LogReg & MLP & CNN\\
%     \hline
%     1\% &  34.09&  31.69&  34.90& 65.78\\
%     5\%  & 27.61 & 31.74 & 35.38 & 68.33\\
%     10\% & 27.07 &  31.59&  34.43& 65.81\\
%     20\% & 28.87 &  30.56&  31.75&  62.54\\
%     50\% &  32.24&   27.37&  27.95& 53.17\\
%     \bottomrule
% \end{tabular}
% \end{table}
% \begin{table}[!t]
% \small
%     \centering
%     \caption{Impact of model size on \toolnameG on {\tt CelebA}~\cite{celeba}.}
%     \label{rq4:table1}
%     \begin{tabular}{c|cc}
%     \toprule
%     Model Size  & {\tt CelebA32} & {\tt CelebA64}\\
%     \hline
%     1.8M& 19.13& 49.27\\
%     4.2M&  17.95& 45.80\\
%     6.3M&  13.94& 40.07\\
%     16.2M&  11.19& \\
%     28.7M&  9.77 & \\
%     \bottomrule
% \end{tabular}
% \end{table}
% \begin{table}[!t]
%     \centering
%     \caption{Impact of model size on \toolnameD on {\tt CIFAR-10}~\cite{cifar10}.}
%     \label{rq4:table2}
%     \begin{tabular}{c|cccc}
%     \toprule
%     Model Size & FID & LogReg & MLP & CNN\\
%     \hline
%     1.8M & 27.61 & 31.74 & 35.38 & 68.33\\
%     4.0M&  24.75&  31.93&  36.75& 70.52\\
%     6.1M &  21.69&  33.31&  36.78& 70.91\\
%     15.7M &  18.34&  32.53&  37.93& 72.13\\
%     27.9M &  18.21&  32.52&  35.51& 72.32\\
%     \bottomrule
% \end{tabular}
% \end{table}
\noindent \textbf{Experiment Design.} This experiment investigates how the selection ratio of selecting pre-training data from the entire public data and the generative model size impact the performance of \toolnameD. The selection ratio is determined by $k_2$. For example, {\tt ImageNet} has 1,000 subsets, each containing nearly the same number of images. When $k_2=10$, it means that 10 subsets will be selected for pre-training, resulting in a selection ratio of 1\%. We explore selection ratios of {1\%, 5\%, 10\%, 20\%, 50\%}. In terms of model size, we consider {1.8M, 4.0M, 6.1M, 15.7M, 27.9M} for {\tt CIFAR-10}, {1.8M, 4.2M, 6.3M, 16.2M, 28.7M} for {\tt CelebA32}, and {2.0M, 4.3M, 6.5M, 17.9M, 31.8M} for {\tt CelebA64}.



\noindent \textbf{Result Analysis.} Figure~\ref{fig:rq4} shows that across all selection ratios, \toolname outperforms the full public dataset (where the selection ratio is 100\%), revealing the effectiveness of our semantic distribution query. As the selection ratio increases, implying more data is used for pre-training, \toolname generally exhibits poorer FID and CA on both {\tt CIFAR-10} and {\tt CelebA}. We believe the reason for this is that only a small portion of {\tt ImageNet} is similar to our sensitive datasets. Pre-training models on a larger number of dissimilar images may distract the models from learning the distribution of similar images, making it more challenging for the models to learn the distribution of the sensitive datasets. However, this trend is more pronounced for {\tt CIFAR-10} than for {\tt CelebA}. This can be attributed to the fact that {\tt CelebA} diverges more from the public dataset {\tt ImageNet}, resulting in fewer opportunities for \toolname to select beneficial data for pre-training. For {\tt CIFAR-10}, the performance of \toolname is notably impacted. Specifically, when the selection ratio is at 1\%, the FID of synthetic images rises compared to that at 5\%. Hence, when there is a significant discrepancy between sensitive and public data, we have the flexibility to select a ratio, which typically outperforms using the entire public dataset. To further investigate this phenomenon, we conduct experiments on another dataset with a larger domain shift from {\tt ImageNet}. The results of these experiments are presented in Appendix G.1 in our full version~\cite{privimage}.

\begin{table}[!t]
\vspace{-5.0pt}
\setlength{\tabcolsep}{3pt}
\small
    \centering
    \caption{The FID and CA of \toolname and three non-private baselines on {\tt CIFAR-10}~\cite{cifar10}, {\tt CelebA32} and {\tt CelebA64}~\cite{celeba} with $\varepsilon=10$.}
    \label{tab:dis1}
    \begin{tabular}{l|cccc|c|c}
    \toprule
    \multirow{3}{*}{Method} & \multicolumn{4}{c|}{{\tt CIFAR-10}} & {\tt CelebA32} & {\tt CelebA64 }\\
    \Xcline{2-7}{0.5pt}
    & \multicolumn{3}{c}{CA (\%)} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID} & \multirow{2}{*}{FID}\\
     \Xcline{2-4}{0.5pt}
     & LR & MLP & CNN & &\\
    \hline
    NonPrivG & 18.2 & 24.7 & 49.8 & 22.5 & 13.6 & 34.7\\
    NonPrivD & 35.8 & 42.2 & 77.1  & 19.8 & 9.01 & 18.0\\
    NonPriv & 37.4 & 45.7 & 86.1 & - & - & -\\
    \hline
    \rowcolor{gray0} \toolnameG & 19.9 & 24.5 & 44.3 & 28.1 & 18.9 & 38.2\\
    \rowcolor{gray0} \toolnameD & 31.7 & 35.4 & 68.3 & 27.6 & 19.1 & 49.3\\
    \bottomrule
\end{tabular}
\vspace{-8.0pt}
\end{table}
In terms of model size, as it increases, \toolname generally achieves superior FID and CA results. However, as the model size becomes significantly larger, the performance gets unstable. For instance, the CA of MLP classifiers trained on synthetic images from \toolname at 27.9M is lower than at 15.7M. Similarly, the CA of LR classifiers from \toolname at 15.7M is below that of 6.1M. These observations suggest that lighter generative models might be better suited for the DP image synthesis task.

\begin{table}[h]
\vspace{-8.0pt}
\setlength{\tabcolsep}{3pt}
    \centering
    \renewcommand\arraystretch{1}
    \begin{tabular}{p{0.95\columnwidth}}
    \Xhline{1.0pt}
         \rowcolor{gray0} \noindent \textbf{Answers to RQ3}: Compared to using the entire public dataset, \toolname achieves superior performance with a selection ratio less than 50\%. As the divergence between public and sensitive data widens, the influence of the selection ratio diminishes gradually. When the generative model comprises fewer than 15M parameters, \toolname produces higher-quality synthesized images with larger models. Whereas, as the parameters increase further, \toolname experiences unstable training.\\
    \Xhline{1.0pt}
    \end{tabular}
\vspace{-8.0pt}
\end{table}

% \noindent \textbf{Answers to RQ4}: Compared to using the entire public dataset, \toolname achieves superior performance with a selection ratio less than 50\%. As the divergence between public and sensitive data widens, the influence of the selection ratio diminishes gradually. Additionally, when the generative model comprises fewer than 15M parameters, \toolname produces higher-quality synthesized images with larger models.







==> Sections/final_rw.tex <==
\section{Related Work}
\label{sec:related_work}

This section explicitly discusses two main types of DP image data synthesis works, including sanitizing generative models through DP-SGD~\cite{dpsgd} and querying DP information of sensitive datasets for synthesis.

\noindent \textbf{Sanitizing Generative Models via DP-SGD.}
Currently, most efforts have focused on applying DP-SGD~\cite{dpsgd} on popular generative models, like GANs~\cite{dpsgd-gan1,dpsgd-gan2,dpsgd-gan4,dpsgd-gan6}, diffusion models~\cite{dpdm,dpldm,dpdm-sota} or variational autoencoders (VAE)~\cite{dp2vae,dps-fvae,lvae}. They introduce noise into gradient calculations during training, ensuring that individual data points do not disproportionately influence the model's learning, thereby offering a degree of privacy protection. 
Diffusion models have shown promise in generating DP image data. For example, PDP-Diffusion~\cite{dpdm-sota} and DPDM~\cite{dpdm} respectively achieve state-of-the-art performance in terms of fidelity and utility of synthetic images, and demonstrate top-tier classification accuracy, both under the setting of with and without the use of a public dataset for pre-training. However, DPDM only achieves synthesis on some naive datasets (e.g. {\tt MNIST}). PDP-Diffusion demands significant computational resources and struggles to produce images with great fidelity and utility on end-user devices for real-world applications~\cite{DPPublicPretraining1}.

\toolname presented in this paper also relies on sanitizing generative models via DP-SGD for DP image synthesis. Different from existing methods, \toolname queries the semantic distribution of the sensitive dataset to select a more compact dataset from the public dataset for pre-training. \toolname enables us to use a lightly parameterized model, while achieving superior synthesis performance.

\noindent \textbf{Querying DP Information for Synthesis.}
Another type of method emphasizes designing a query function to extract valuable features from a sensitive dataset~\cite{dp-mepf,dp-merf,pearl,api,dp-kernel,dp-ntk}. These features exhibit low sensitivity and aid in obtaining pertinent information for synthesis. 
% We query the marginal of tabular dataset whose sensitivity is 1~\cite{privsyn}. When incorporating Gaussian noise, the noisy features can be viewed as a target. We simply need to devise a method (e.g., GANs) to produce a synthetic dataset with features closely resembling this target~\cite{dp-merf,pearl,dp-mepf}. 
We will next introduce the various feature query functions without delving into the generation process.

Harder et al. presented DP-MERF~\cite{dp-merf}, a method that represents the sensitive dataset using random features like Fourier features. Meanwhile, Seng et al.~\cite{pearl} suggested substituting the random feature with a characteristic function, which offers improved generalization capability. Harder et al. introduced DP-MEPF~\cite{dp-mepf}, a method that leverages public data to extract perceptual features. Specifically, they represent each image as a feature vector using an encoder pre-trained on public datasets, such as {\tt ImageNet}~\cite{imagenet}. These methods, however, fall short in comparison to DP-SGD~\cite{dpsgd} in term of generated images qualification, especially for more colorful dataset (e.g., {\tt CIFAR-10}~\cite{cifar10}). Recently, DPSDA~\cite{api} proposed to utilize foundation model APIs of powerful generative models trained on public datasets, such as DALLE-2~\cite{dalle2}, Stable Diffusion~\cite{StableDiffusion}, and GPT3/4~\cite{gpt3,gpt4}. Although this method achieves results comparable to the SOTA~\cite{dpdm-sota}, DPSDA heavily depends on two open-source APIs, RANDOM-API and VARIATION-API, which may not be available in some scenarios, especially for the VARIATION-API.
